Lite2Relight: 3D-aware Single Image Portrait Relighting

Achieving photorealistic 3D view synthesis and relighting of human portraits is pivotal for advancing AR/VR applications. Existing methodologies in portrait relighting demonstrate substantial limitations in terms of generalization and 3D consistency, coupled with inaccuracies in physically realistic lighting and identity preservation. Furthermore, personalization from a single view is difficult to achieve and often requires multiview images during the testing phase or involves slow optimization processes. This paper introduces Lite2Relight, a novel technique that can predict 3D consistent head poses of portraits while performing physically plausible light editing at interactive speed. Our method uniquely extends the generative capabilities and efficient volumetric representation of EG3D, leveraging a lightstage dataset to implicitly disentangle face reflectance and perform relighting under target HDRI environment maps. By utilizing a pre-trained geometry-aware encoder and a feature alignment module, we map input images into a relightable 3D space, enhancing them with a strong face geometry and reflectance prior. Through extensive quantitative and qualitative evaluations, we show that our method outperforms the state-of-the-art methods in terms of efficacy, photorealism, and practical application. This includes producing 3D-consistent results of the full head, including hair, eyes, and expressions. Lite2Relight paves the way for large-scale adoption of photorealistic portrait editing in various domains, offering a robust, interactive solution to a previously constrained problem. Project page: https://vcai.mpi-inf.mpg.de/projects/Lite2Relight/

==> tex_fig/method/losst.tex <==
\begin{figure}
\centering
\newcommand{\mywidth}{0.8}
\begin{tikzpicture}[every node/.style={inner sep=0,outer sep=0}]
\matrix[matrix of nodes, nodes={anchor=center}, row sep=1mm]{
 \includegraphics[trim=0em 0em 0em 1em, clip=true, width=\mywidth\linewidth]{figures/TripletLoss.png}
%&
% GT  & Single-view & Multi-view 
\\
};
\end{tikzpicture}
\caption{Triplet Loss: }
\label{fig:triplet_loss}
\end{figure}

==> tex_tab/abln_additional_metrics.tex <==
\begin{table}[ht]
\centering
\caption{\textbf{Quantitative Results: Ablation Study: Additional Metrics.} We report LPIPS, RMSE and DISTS metrics in addition to SSIM, landmarks distance (LD), and PSNR on the test data of lightstage, where  subjects are relit under novel viewpoints.} 
\begin{tabular}{lcccccc}
\hline 
           & LPIPS$\downarrow$ & RMSE$\downarrow$ & DISTS$\downarrow$  \\ \hline
PhotoaApp  & 0.4163 & 0.1988 & 0.2031  \\
NeRFFaceLighting & 0.2966 & 0.2905 & 0.2409  \\ \hline
\OurMethod &  \textbf{0.2493}& \textbf{0.1841} & \textbf{0.1718} \\ \hline
\end{tabular}
\label{tab:abln_additional_metrics}
\end{table}

==> tex_tab/abln_n_subjects.tex <==
\begin{table}[ht]
\centering
\caption{\textbf{Quantitative Results: Ablation Study: Number of Subjects.} We report SSIM, landmarks distance (LD), and PSNR on the test data of lightstage, where  subjects are relit under novel viewpoints.} 
\begin{tabular}{lcccc}
\hline
           & SSIM $\uparrow$ & LD $\downarrow$ & PSNR $\uparrow$ \\ \hline
Subjects = 10  & 0.829 & 10.24 & 28.26 \\
Subjects = 50  & 0.829 & 9.61 & 28.31 \\\hline
Subjects = 250 &  \textbf{0.834} & \textbf{9.76} &\textbf{28.33} \\ \hline
\end{tabular}
\label{tab:abln_n_subjects}
\end{table}

==> tex_tab/abln_n_views.tex <==
\begin{table}[ht]
\centering
\caption{\textbf{Quantitative Results: Ablation Study: Number of Viewpoints.} We report SSIM, landmarks distance (LD), and PSNR on the test data of lightstage, where  subjects are relit under novel viewpoints.} 
\begin{tabular}{lcccc}
\hline
           & SSIM $\uparrow$ & LD $\downarrow$ & PSNR $\uparrow$ \\ \hline
Views = 1  & 0.831 & 10.45 & 28.31 \\
Views = 4  & 0.834 & 10.26 & 28.30 \\
Views = 8  & 0.834 & 10.1 & 28.31 \\ \hline
Views = 2 &  \textbf{0.834} & \textbf{9.76} &\textbf{28.33} \\ \hline
\end{tabular}
\label{tab:abln_n_views}
\end{table}


==> tex_tab/related_works.tex <==
% \begin{table}[]
% \centering
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
%           & Monocular & Generalize & 3D Consistent & Light Consitency & Real-Time \\ \hline
% PhotoApp  & Yes       & Yes        & No            & No               & Yes       \\ \hline
% MEGANE    & No        & Yes        & Yes           & Yes              & Yes       \\ \hline
% LumiGAN   & Yes       & Yes        & Yes           & No               & No        \\ \hline
% TR Avatar & No        & No         & Yes           & Yes              & Yes       \\ \hline
% VoRF      & Yes       & Yes        & Yes           & Yes              & No        \\ \hline
% Ours      & Yes       & Yes        & Yes           & Yes              & Yes       \\ \hline
% \end{tabular}
% \caption{Summary}
% \label{tab:related_works}
% \end{table}
\begin{table*}[]
% \small 
% \setlength{\tabcolsep}{3pt}
% \centering
\caption{Our approach achieves a mix of novel capabilities for portrait image editing such as 3D consistent pose synthesis, physically accurate relighting, semantic editing and an efficient feedforward encoder-based inference pipeline that enables real-time performance.}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
          & Monocular & Novel Identity & 3D Consistency & Physical Relighting & Real-Time & Semantic Editing \\ \hline
EG3D~\cite{mallikarjun2021photoapp}  & Yes       & Yes        & Yes            & No               & Yes   & Yes     \\ \hline
PhotoApp~\cite{mallikarjun2021photoapp}  & Yes       & Yes        & No            & No               & Yes   & No     \\ \hline
% MEGANE~\cite{megane}    & No        & Yes        & Yes           & Yes              & Yes & No      \\ \hline
LumiGAN~\cite{deng2023lumigan}   & Yes       & Yes        & Yes           & No               & No & No       \\ \hline
NeLF~\cite{sun2021nelf} & No        & No         & Yes           & Yes              & Yes    & No   \\ \hline
VoRF~\cite{prao2022vorf}      & Yes       & Yes        & Yes           & Yes              & No     & No   \\ \hline
Ours      & Yes       & Yes        & Yes           & Yes              & Yes    & Yes   \\ \hline
\end{tabular}
\end{center}
\label{tab:related_works}
\end{table*}
